Two-Stage Decoupling Framework for Variable-Length Glaucoma Prognosis

Glaucoma is one of the leading causes of irreversible blindness worldwide. Glaucoma prognosis is essential for identifying at-risk patients and enabling timely intervention to prevent blindness. Many existing approaches rely on historical sequential data but are constrained by fixed-length inputs, limiting their flexibility. Additionally, traditional glaucoma prognosis methods often employ end-to-end models, which struggle with the limited size of glaucoma datasets. To address these challenges, we propose a Two-Stage Decoupling Framework (TSDF) for variable-length glaucoma prognosis. In the first stage, we employ a feature representation module that leverages self-supervised learning to aggregate multiple glaucoma datasets for training, disregarding differences in their supervisory information. This approach enables datasets of varying sizes to learn better feature representations. In the second stage, we introduce a temporal aggregation module that incorporates an attention-based mechanism to process sequential inputs of varying lengths, ensuring flexible and efficient utilization of all available data. This design significantly enhances model performance while maintaining a compact parameter size. Extensive experiments on two benchmark glaucoma datasets:the Ocular Hypertension Treatment Study (OHTS) and the Glaucoma Real-world Appraisal Progression Ensemble (GRAPE),which differ significantly in scale and clinical settings,demonstrate the effectiveness and robustness of our approach.

==> table.tex <==
\begin{table}[htbp]
   \centering
   \setlength{\tabcolsep}{5pt}
   \caption{The results on OHTS dataset}
   \begin{tabular}{lccccc}
       \toprule
       & $\Delta t$ & ACC & AUC & PARAMs & Patient Num. \\ 
       \midrule
       ResNet50 & -- & 0.880 (±0.010) & 0.780 (±0.020) & 23,512,130 & 3167 \\ 
       \midrule
       \multirow{4}{*}{LSTM} 
       & 1 & 0.861 (±0.082) & 0.704 (±0.118) & \multirow{4}{*}{25,869,890} & 3167 \\
       & 2 & 0.884 (±0.211) & 0.834 (±0.115) &  & 3038 \\
       & 3 & 0.892 (±0.140) & 0.759 (±0.317) &  & 2888 \\
       & 4 & 0.898 (±0.139) & 0.863 (±0.214) &  & 2763 \\
       \midrule
       Ours & -- & 0.907 (±0.008) & 0.931 (±0.013) & 4,136,452 & 3167 \\
       \bottomrule
   \end{tabular}
   \label{tab:ohts_results}
\end{table}


\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{5pt}
\caption{The results on the GRAPE dataset.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
 & $\Delta t$ & \multicolumn{3}{c}{ACC} & \multicolumn{3}{c}{AUC} & \multirow{2}{*}{Patient Num.} \\ 
 \cmidrule(rl){3-5} \cmidrule(rl){6-8}
 &  & PLR2 & PLR3 & MD & PLR2 & PLR3 & MD &  \\ 
 \midrule
ResNet50 & -- & 0.750 (±0.015) & 0.910 (±0.012) & 0.810 (±0.013) & 0.710 (±0.057) & 0.800 (±0.076) & 0.730 (±0.118) & 263 \\ 
\midrule
\multirow{2}{*}{LSTM} 
& 1 & 0.774 (±0.014) & 0.925 (±0.011) & 0.943 (±0.012) & 0.733 (±0.238) & 0.744 (±0.117) & 0.519 (±0.419) & 263 \\
& 2 & 0.775 (±0.013) & 0.945 (±0.010) & 0.905 (±0.011) & 0.481 (±0.219) & 0.666 (±0.188) & 0.882 (±0.016) & 196 \\
\midrule
Ours & -- & 0.896 (±0.009) & 0.951 (±0.008) & 0.911 (±0.009) & 0.866 (±0.150) & 0.956 (±0.017) & 0.917 (±0.058) & 263 \\ 
\bottomrule
\end{tabular}
}
\label{tab:grape_results}
\end{table}

